Probabilistic Iterative LQR for Short Time Horizon MPC

Optimal control is often used in robotics for planning a trajectory to achieve some desired behavior, as expressed by the cost function. Most works in optimal control focus on finding a single optimal trajectory, which is then typically tracked by another controller. In this work, we instead consider trajectory distribution as the solution of an optimal control problem, resulting in better tracking performance and a more stable controller. A Gaussian distribution is first obtained from an iterative Linear Quadratic Regulator (iLQR) solver. A short horizon Model Predictive Control (MPC) is then used to track this distribution. We show that tracking the distribution is more cost-efficient and robust as compared to tracking the mean or using iLQR feedback control. The proposed method is validated with kinematic control of 7-DoF Panda manipulator and dynamic control of 6-DoF quadcopter in simulation.

==> sections/related_works.tex <==
\section{Related Work}
\label{sec:related_works}

\subsection{Optimal control for planning}
\label{sec:optimal_planning}

Optimal control is often used in robotics for planning state trajectories that maximize certain performance characteristics, e.g., reaching the goal in minimum time, avoiding obstacles, consuming minimum energy, or moving with limited velocities/accelerations. A long horizon formulation allows us to consider future events that enable more stable behaviours and better prediction. Robinson \emph{et al.} generate optimal trajectories for 32 quadcopters in a constrained space. In~\cite{Kajita2003}, Kajita \emph{et al.} use optimal control for biped walking generation using the linear inverted pendulum model. Caron and Kheddar~\cite{Caron2016} extend this to multi contact locomotion. 
Ponton \emph{et al.} plan the optimal centroidal dynamics trajectory in~\cite{Ponton2018}. In~\cite{Winkler2018}, the gait sequence, step timings, footholds, and swing-leg motions are also included as the optimization variables. Whole-body motion planning has been done in recent work~\cite{Budhiraja2019},~\cite{Mastalli}. Optimal control has also been used in the context of visual servoing~\cite{Paolillo2020}. 

These work often involves a long horizon to be able to produce complex movements that consider future events or desired behaviour, such as obstacle avoidance~\cite{Paolillo2020} or momentum control~\cite{Budhiraja2019}. The trajectory generation is often one part of a larger control strategy, where the trajectory is then tracked using some other simpler controllers. For example, Carpentier \emph{et al.} use a second-order inverse kinematics to track the generated centroidal trajectory. In ~\cite{Paolillo2020}, a short time horizon MPC is used in real time. While technically the long time horizon optimal control can be used in MPC fashion, this requires a long computation time, making such approach often infeasible. 


\subsection{Probabilistic formulation of optimal control}
\label{sec:prob_oc}

Most work in optimal control focus on finding only one optimal solution. However, optimal control problem can also be viewed as probabilistic inference problem, allowing approximate inference techniques to be applied for solving an optimal control problem more efficiently. In this case, the output will be the probability distribution of the control trajectory that minimize the cost. In ~\cite{Kappen2012}, Kappen \emph{et al.} consider the optimal control as minimizing Kullback-Leibler (KL) divergence. The optimal control solution is the product of the free dynamics and the exponentiated cost (i.e. the exponent of the cost function is considered as an unnormalized probability distribution). Toussaint~\cite{Toussaint2009} show that using an approximate inference method (similar to expectation propagation) to solve an optimal control problem results in an algorithm that is similar to iterative Linear Quadratic Gaussian (iLQG).  

Although the probabilistic formulation has been investigated, most of them concentrate on improving the efficiency, and not many works actually use the probabilistic solution, except in Guided Policy Search (GPS~\cite{Levine2013} ) where the probabilistic distribution of iLQR solution is used as a guiding distribution for reinforcement learning. In this work, we show that we can obtain the probabilistic distribution of both control and state trajectories efficiently from an iterative LQR solver. The distribution is then tracked using a short time horizon MPC. We show that tracking a full probability distribution improves the tracking performance as compared to tracking only the mean. 
